Speech-MASSIVE: A Multilingual Speech Dataset for SLU and Beyond

We present Speech-MASSIVE, a multilingual Spoken Language Understanding (SLU) dataset comprising the speech counterpart for a portion of the MASSIVE textual corpus. Speech-MASSIVE covers 12 languages from different families and inherits from MASSIVE the annotations for the intent prediction and slot-filling tasks. Our extension is prompted by the scarcity of massively multilingual SLU datasets and the growing need for versatile speech datasets to assess foundation models (LLMs, speech encoders) across languages and tasks. We provide a multimodal, multitask, multilingual dataset and report SLU baselines using both cascaded and end-to-end architectures in various training scenarios (zero-shot, few-shot, and full fine-tune). Furthermore, we demonstrate the suitability of Speech-MASSIVE for benchmarking other tasks such as speech transcription, language identification, and speech translation. The dataset, models, and code are publicly available at: https://github.com/hlt-mt/Speech-MASSIVE

==> tables/apdx/slot_cer.tex <==
\begin{table}[!htp]\centering
\resizebox{\linewidth}{!}{

\begin{tabular}{c|cc|cc}
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{zero-shot}}       & \multicolumn{2}{c}{\textbf{few-shot}}         \\
lang                  & E2E SLU (En)          & E2E SLU (Fr)          & E2E SLU (En)          & E2E SLU (Fr)          \\ \hline
ar-SA                 & 10.23 ± 2.64          & 16.41 ± 1.33          & 36.27 ± 0.69          & 38.58 ± 0.67          \\
de-DE                 & 50.56 ± 1.95          & 54.12 ± 1.09          & 59.56 ± 0.85          & 62.12 ± 0.54          \\
es-ES                 & 47.51 ± 0.55          & 50.38 ± 0.80          & 55.04 ± 2.03          & 58.39 ± 0.31          \\
fr-FR                 & 37.17 ± 2.2           & 62.30 ± 0.47          & 49.93 ± 0.29          & 62.31 ± 0.22          \\
hu-HU                 & 18.54 ± 1.51          & 22.61 ± 0.67          & 42.01 ± 0.24          & 46.12 ± 0.17          \\
ko-KR                 & 23.38 ± 3.55          & 27.37 ± 1.78          & 41.43 ± 0.89          & 43.30 ± 1.11          \\
nl-NL                 & 44.57 ± 0.58          & 44.88 ± 0.45          & 55.90 ± 0.14          & 57.68 ± 0.30          \\
pl-PL                 & 35.93 ± 2.55          & 40.74 ± 1.07          & 51.53 ± 1.29          & 55.20 ± 0.24          \\
pt-PT                 & 32.72 ± 1.31          & 40.12 ± 2.22          & 48.48 ± 1.46          & 51.13 ± 0.67          \\
ru-RU                 & 41.10 ± 3.42          & 48.70 ± 1.05          & 57.40 ± 0.73          & 59.45 ± 0.47          \\
tr-TR                 & 24.44 ± 2.76          & 29.51 ± 1.09          & 45.95 ± 0.88          & 48.59 ± 0.99          \\
vi-VN                 & 12.01 ± 2.04          & 21.98 ± 3.06          & 44.40 ± 1.50          & 50.26 ± 0.56          \\ \hline
\textbf{avg}          & \textbf{31.51 ± 1.32} & \textbf{36.07 ± 1.04} & \textbf{48.99 ± 1.50} & \textbf{51.89 ± 1.50}
\end{tabular}
}
\caption{\bl{TBU : Slot value CER for all the settings.}}
\label{tab:apdx_slot_value_cer}
\end{table}

==> tables/apdx/slot_type_f1.tex <==
\begin{table}[!htp]\centering
\resizebox{\linewidth}{!}{

\begin{tabular}{c|cc|cc}
\multicolumn{1}{l|}{} & \multicolumn{2}{c|}{\textbf{zero-shot}}       & \multicolumn{2}{c}{\textbf{few-shot}}         \\
lang                  & E2E SLU (En)          & E2E SLU (Fr)          & E2E SLU (En)          & E2E SLU (Fr)          \\ \hline
ar-SA                 & 10.23 ± 2.64          & 16.41 ± 1.33          & 36.27 ± 0.69          & 38.58 ± 0.67          \\
de-DE                 & 50.56 ± 1.95          & 54.12 ± 1.09          & 59.56 ± 0.85          & 62.12 ± 0.54          \\
es-ES                 & 47.51 ± 0.55          & 50.38 ± 0.80          & 55.04 ± 2.03          & 58.39 ± 0.31          \\
fr-FR                 & 37.17 ± 2.2           & 62.30 ± 0.47          & 49.93 ± 0.29          & 62.31 ± 0.22          \\
hu-HU                 & 18.54 ± 1.51          & 22.61 ± 0.67          & 42.01 ± 0.24          & 46.12 ± 0.17          \\
ko-KR                 & 23.38 ± 3.55          & 27.37 ± 1.78          & 41.43 ± 0.89          & 43.30 ± 1.11          \\
nl-NL                 & 44.57 ± 0.58          & 44.88 ± 0.45          & 55.90 ± 0.14          & 57.68 ± 0.30          \\
pl-PL                 & 35.93 ± 2.55          & 40.74 ± 1.07          & 51.53 ± 1.29          & 55.20 ± 0.24          \\
pt-PT                 & 32.72 ± 1.31          & 40.12 ± 2.22          & 48.48 ± 1.46          & 51.13 ± 0.67          \\
ru-RU                 & 41.10 ± 3.42          & 48.70 ± 1.05          & 57.40 ± 0.73          & 59.45 ± 0.47          \\
tr-TR                 & 24.44 ± 2.76          & 29.51 ± 1.09          & 45.95 ± 0.88          & 48.59 ± 0.99          \\
vi-VN                 & 12.01 ± 2.04          & 21.98 ± 3.06          & 44.40 ± 1.50          & 50.26 ± 0.56          \\ \hline
\textbf{avg}          & \textbf{31.51 ± 1.32} & \textbf{36.07 ± 1.04} & \textbf{48.99 ± 1.50} & \textbf{51.89 ± 1.50}
\end{tabular}
}
\caption{Slot type F1 for all the settings.}
\label{tab:apdx_slot_type_f1}
\end{table}
